Teledrive: An Embodied AI based Telepresence System

This article presents Teledrive, a telepresence robotic system with embodied AI features that empowers an operator to navigate the telerobot in any unknown remote place with minimal human intervention. We conceive Teledrive in the context of democratizing remote care-giving for elderly citizens as well as for isolated patients, affected by contagious diseases. In particular, this paper focuses on the problem of navigating to a rough target area (like bedroom or kitchen) rather than pre-specified point destinations. This ushers in a unique AreaGoal based navigation feature, which has not been explored in depth in the contemporary solutions. Further, we describe an edge computing-based software system built on a WebRTC-based communication framework to realize the aforementioned scheme through an easy-to-use speech-based human-robot interaction. Moreover, to enhance the ease of operation for the remote caregiver, we incorporate a person following feature, whereby a robot follows a person on the move in its premises as directed by the operator. Moreover, the system presented is loosely coupled with specific robot hardware, unlike the existing solutions. We have evaluated the efficacy of the proposed system through baseline experiments, user study, and real-life deployment.

==> abstract.tex <==
%\abstract{The goal of any cutting-edge robotic telepresence system is to enable a virtual presence of the remote participant through real-time mobility of the robotic avatar while interacting with the remote environment over multimedia conferencing. Hence, smart navigation is an essential feature of such robot systems. However, existing telepresence systems do not support inbuilt cognitive navigation, based on semantic scene analysis. This paper presents `Teledrive', a telepresence robotic system empowered with embodied AI features. The whole system has been conceived in the context of remote `care-giving' for elderly citizens as well as for isolation patients in a pandemic situation. In particular, this paper focuses on the `AreaGoal' problem whereby the robot needs to reach a target area based on the visual cues. To the best of our knowledge, this is the first work dealing with `AreaGoal' task. This paper provides a unique solution to the problem based on in situ intelligent visual semantic mapping of the live scene capture by the robot. It further presents the Edge-centric software system architecture of Teledrive comprising a speech recognition based HRI system, the navigation module and the real-time WebRTC based communication framework that holds the entire system together. The paper establishes the efficacy of the proposed smart navigation algorithm through benchmarking experiments and finally concludes by describing a real-life deployment of the system.}

\abstract{The goal of any robotic telepresence system is to enable a virtual presence of the remote participant through real-time mobility of the robotic avatar while interacting with the remote environment over multimedia conferencing. Hence, smart navigation is an essential feature of such robot systems. However, existing telepresence systems lack semantic navigation capability that requires minimal user intervention. This article presents `Teledrive', a telepresence robotic system with embodied AI features that empowers a user to navigate the robot in any unknown remote place. We conceive Teledrive in the context of remote `care-giving' for elderly citizens as well as for isolation patients in a pandemic situation. In particular, this paper focuses on the `AreaGoal' problem whereby the robot needs to reach a target area based on visual cues. To the best of our knowledge, this is the first work on the `AreaGoal' embodied AI task. This paper provides a unique solution to the problem based on in situ intelligent visual semantic mapping of the live scene captured by the robot. Additionally, we describe a novel edge-centric software system architecture, which comprises a speech recognition-based human-robot interaction capability, the navigation module, and the real-time WebRTC based communication framework. We further present person following methodology and user interface studies. We evaluate the efficacy of the proposed smart navigation algorithm through benchmarking experiments and a real-life deployment of the system.}


==> comparison.tex <==
%\begin{landscape}
\begin{table*}
    \centering
    \caption{Comparison of features in existing telepresence systems.}
    \label{tab:comparison_variations}
    \rotatebox{90}{
    \begin{tabular}{|p{2cm}|l|l|p{1.1cm}|p{0.55cm}|l|p{0.5cm}|p{0.85cm}|l|p{1.5cm}|p{1.05cm}|l|p{0.8cm}|p{1cm}|l|}
    \hline
        Features & Teledrive & Double 3 & ENRICH ME & Amy A3 & Kuby & Ava 500 & PadBot P3 & Vgo & Ohmni SuperCam & BotEyes Pad & Giraff & Beam Pro & FURo-I home & Temi \\ \hline
        \nohyphens{Platform independence} & y & n & n & n & n & n & n & n & n & n & n & n & n & n \\ \hline
        \nohyphens{Browser\;\;\;\;\;\;\; GUI} & y & y & n & n & n & n & n & y & y & y & n & n & n & n \\ \hline
        \nohyphens{Manual navigation} & y & y & y & y & n & y & y & y & y & y & y & y & y & n \\ \hline
        \nohyphens{AR goal based navigation} & y & y & n & y & n & n & n & n & n & n & n & n & n & y \\ \hline
        \nohyphens{Map based navigation} & y & n & y & n & n & y & n & n & n & n & n & n & n & y \\ \hline
        \nohyphens{Area goal based navigation} & y & n & n & n & n & n & n & n & n & n & n & n & n & n \\ \hline
        \nohyphens{Speech based navigation} & y & n & n & n & n & n & n & n & n & n & n & n & n & y \\ \hline
        \nohyphens{Information mashup} & y & n & n & n & n & n & n & n & n & n & n & n & n & n \\ \hline
        \nohyphens{Speaker localization} & y & n & n & n & y & n & n & n & n & n & n & n & n & n \\ \hline
        \nohyphens{Face identification} & y & n & y & y & n & n & y & n & n & n & n & n & y & y \\ \hline
        \nohyphens{Person following} & y & n & n & n & n & n & n & n & n & n & n & n & n & y \\ \hline
        \nohyphens{Multi-party federated control} & y & n & n & n & n & n & n & n & n & n & n & n & n & n \\ \hline
        \nohyphens{Automatic map generation} & y & n & y & n & n & n & n & n & n & n & n & n & n & y \\ \hline
        \nohyphens{Dialogue based disambiguation} & y & n & n & n & n & n & n & n & n & n & n & n & n & n \\ \hline
    \end{tabular}
    }
\end{table*}
%\end{landscape}

% \centering
% \begin{table}[h]
% \begin{tabular}{|p{1.5cm}|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline 
% Features & Teledrive & Double 3 & ENRICHME & Amy A3 & Kuby & AVA 500 & PadBot P3 & Vgo & Ohmni SuperCam & BotEyes-Pad & Giraff & Beam Pro & FURo-I home & Temi\\
% \hline 
% Platform independence & yes &  &  &  &  &  &  &  &  &  &  &  &  &
% \\ \hline
% Browser GUI & yes &  &  &  &  &  &  &  &  &  &  &  &  &
% \\ \hline
% Manual navigation & yes &  &  &  &  &  &  &  &  &  &  &  &  &
% \\ \hline
% Air-goal navigation & yes &  &  &  &  &  &  &  &  &  &  &  &  &
% \\ \hline
% Map-based navigation & yes &  &  &  &  &  &  &  &  &  &  &  &  & 
% \\ \hline
% Area goal based navigation & yes &  &  &  &  &  &  &  &  &  &  &  &  & 
% \\ \hline
% Speech-based navigation & yes &  &  &  &  &  &  &  &  &  &  &  &  &
% \\ \hline
% Information mashup & yes &  &  &  &  &  &  &  &  &  &  &  &  &
% \\ \hline
% Speaker localization & yes &  &  &  &  &  &  &  &  &  &  &  &  & 
% \\ \hline
% Face identification & yes &  &  &  &  &  &  &  &  &  &  &  &  & 
% \\ \hline
% Person following & yes &  &  &  &  &  &  &  &  &  &  &  &  & 
% \\ \hline
% Multi-party federated control & yes &  &  &  &  &  &  &  &  &  &  &  &  &
% \\ \hline
% Automatic map generation & yes &  &  &  &  &  &  &  &  &  &  &  &  & \\ \hline
% Dialogue-based disambiguation & yes &  &  &  &  &  &  &  &  &  &  &  &  &
% \\ \hline
% \end{tabular}
% \caption{Comparison of telepresence features}
% \label{tab:comparison_variations}
% \end{table}


==> dialogue.tex <==
\section{Cognitive Dialogue exchange}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/telepresence_hri_archi.pdf}
    \caption{Embedding of human-robot interaction mechanism into \system.}
    \label{fig:archi_hri}
\end{figure*}

In a telepresence system, the robotic platform is primarily used to interact with the human beings. However, occasionally the master can control the robot and instruct it to perform a set of tasks/activities. This includes navigate to a location with the(indoor) environment, move closer to or further away from an object/person, tilt the camera, zoom onto some object, etc. However, instead of manually controlling the robot through a continuous set of control commands, autonomous action by the robot based on high level command is very much desirable. This requires a robust human-robot interaction module.

Figure~\ref{fig:archi_hri} depicts the HRI module embedded with our teledrive system. Since speech interface is the most intuitive and user friendly way to interact with a robot, teledrive also supports a speech based task instruction to the robot. However, most of the time what the master says is meant for the remote audience. To distinguish the control instruction for the robot and ordinary speech, we devised a protocol of prefixing the control instruction with a command word. This is common for many personal assistant systems where a wake ward is spoken first before giving any instruction to the assistant. Now, whenever an audio signal is received by the robot, which is detected using a voice activity detection (VAD) module, it is further processed for the command word detection. If there is no command word, no further action is taken. On the other hand, if the command word is defected, the command mode is activated. The command word is detected using a CNN based binary classifier. The model takes any audio chunk and outputs whether the audio chunk contains the command word or not.
In the command mode, the received audio is recorded locally on the robot until a significant silence is detected by the VAD, which signifies end of instruction. Then, the recorded audio is transmitted to the robot-edge for further processing. At the robot edge, first, the audio is translated to text. For this, we use wav2vec based automated speech recognition (ASR) model, which is trained using a transformer based deep neural network~\cite{schneider2019wav2vec}. We use the pretrained model provided by the Facebook AI Research. Then, the textual instruction is passed to a task identification module. This module identifies the task type and the parameter(s) from the natural language instruction. If the task understanding is successful, a planning problem is formulated using the PDDL format. A execution plan is generated using the FF-planner that maps subtasks to robot's action level API. The execution plan is communicated to the robot, where the plan is executed through API calls. At this point, the robot exits from the command mode. In case the robot-edge fails to decode the task instruction, it generates a query for the master that is passed onto the master's devices through the robot. For task understanding and query generation we have used the ``Task Conversational Agent For Robots'' (TCAR)~\cite{pramanick2019enabling, pramanick2019your}.



==> intro.tex <==
\section{Introduction}

%The advent of low cost mobile robotic platform has seen a surge in usage of robots in our daily surroundings. The utility of a mobile robot expanded from personal usage to industry, shop floor, healthcare and office. Additionally, robots are equally used in collocated and remote setup. As a result, a diverse set of applications have emerged where a mobile robotic platform is used by a remote user to interact with the environment where the robot is located. These applications can be broadly categorized as telepresence and teleoperation. In the first category, the robot is essentially a mobile platform where it can move within the environment based on the remote user's command. In the second category, a robot can perform a set of activities based on the remote user's instruction. A telepresence robot may or may not perform any manipulation (actuation) activity, whereas a teleoperation robot may or may have mobility capability. In this article, we primarily focus on a telepresence robotic system.

The advent of low-cost mobile robotic platforms has seen a surge in the usage of robots in our daily surroundings. The utility of a mobile robot expanded from industry to healthcare, shop floor, office, home, etc. Additionally, the usage of modern robots has expanded from in-house operations to remote operations. As a result, a diverse set of applications have emerged where a mobile robotic platform is used by a remote user to interact with the environment where the robot is located. These applications can be broadly categorized as telepresence and teleoperation. In the first category, the robot is essentially a mobile platform where it can move within the environment based on the remote user’s command/intent. In the second category, a robot can perform a set of real-time actuation based on the remote user’s instruction. Of course, there can be a hybrid category where a mobile teleoperation robot can be used for telepresence purposes as well. In this article, we primarily focus on a telepresence robotic system in the context of remote caregiving.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/intro_use_case.png}
    \caption{Illustration of `Teledrive' as an use case in isolation center.}
    \label{fig:pointNav}
\end{figure}

% \subsection{Motivation and Contribution}
\textbf{Motivation.}
% the story how a sick patient can take help of the telepresence. stakeholders: doctor, patient, nurse, medical body / operations
%\subsection{Major Contributions}
The prevalent pandemic situation demands `social distancing' as the new normal. Yet careful monitoring of patients in isolation must be taken care of without risking the lives of `caregivers'. Even without the pandemic, there is a shortage of caregivers in different parts of the world, which is exposed to be acute during the pandemic. The availability of caregiver service must be done in a democratized manner such that individual care is possible for geographically distant individuals. A telepresence robot can address part of this issue. However, the major hindrance in the wider deployment of telepresence systems is the ease of use, particularly for a non-expert user. Existing telepresence systems, provide a manual navigation capability~\cite{}, which is often cumbersome for a user in a non-familiar environment. Moreover, manual navigation requires continuous user intervention to move the remote robot from place to place within the remote environment. Additionally, existing telepresence systems are co-developed with the robot hardware~\cite{}, which makes it difficult for enhancement, particularly by third-party developers. This is mainly done due to the resource constraints existing on the robot hardware. As a result, hardware-independent software development should also be agnostic of resource constraints.

\textbf{Problem statement.}
A telepresence system typically maintains a real-time connection with an application at the caregiver’s~\footnote{Caregiver is mentioned in a remote healthcare context, who is nothing but a remote user in a general sense.} end and acts as an Avatar of the caregiver at the patient’s premise. The caregiver must navigate the patient’s premise in real-time through the Avatar based on the audio-visual feedback as part of the ongoing real-time multimedia chat~(Fig.~\ref{fig:areanav_intro}). In most of the systems, the robot Avatar is maneuvered by the remote caregiver through manual instructions using on-screen navigation buttons, joystick, keyboard, etc. However, in an unknown premise (in the case of a tele-doctor), it would be too tedious for the caregiver to manually navigate the robot to the patient’s location. Hence, we conceive a system such that the caregiver can provide a remote verbal instruction to the robot to navigate near a desired location inside the room (e.g., `bedroom'). This can be further extended wards in isolation centers. The speech-based human-robot interaction (HRI) increases the usability and acceptability of the robot. Recent developments on semantic map building and speech-based HRI can be used as a building block for a telepresence robot software system. However, modern neural network-based systems provide a highly accurate outcome at the expense of higher computing and memory resources, which become scarce when multiple neural network (NN) models are to run the robot for different tasks. Thus, a software architecture is required that can facilitate various NN models to be integrated with the system without compromising on accuracy.

\textbf{Approach.}
%Teledrive uses a semantic map generation model that creates 
Based on the in-situ analysis of the semantic mapping derived from the live captured frames, the robot is able to move to a position near to the intended location. Once the robot reaches `near' that position, the caregiver can take manual control and perform finer control through on-screen navigation buttons. The scenario is depicted in Fig. 1. The robot is connected with the caregiver’s PDA over the Internet through a WebRTC based communication protocol. The robot is at the entrance of the patient’s premises. The old patient is in the bedroom. The caregiver verbally instructs the robot to navigate to the bedroom. Once the robot is able to locate itself around the bedroom, the caregiver can manually lead the robot to the bed where the old patient is waiting.
This motivates us to develop a navigation capability along with a software architecture that makes it platform-independent.

\textbf{Contributions.}
The prime contributions of this article are two folds. Firstly, we describe the cognitive navigation problem, especially in the light of navigating the `AreaGoal'. We show the efficacy of our `AreaGoal' navigation system by results derived from benchmark experiments. Secondly, we present the unique software system architecture comprising the speech-based HRI, the navigation module, and the real-time WebRTC based communication framework. The software architecture supports adding any further AI-based software modules. The communication framework holds the entire system together to serve multiple use cases such as the `caregiver' telepresence scenario.

\input{Comparison}

The overall organization of the paper is as follows. Section ~\ref{related_work} provides a survey of the state-of-the-art telepresence systems along with different evaluation metrics of a cognitive navigation system. Then it further describes the different types of cognitive navigation components. In section~\ref{}, we present the software system architecture with a description of each major sub-component. Section~\ref{} describes the experimental evaluation of the `AreaGoal' navigation. Section~\ref{} describes a practical implementation of the system on a commercial telepresence robot hardware. Finally, we conclude the article in section~\ref{} along with the future research endeavors.

==> related.tex <==
\section{Related Work}
\label{related_work}

% \input{Comparison}

There has been a significant amount of work done in the telepresence scenario \cite{melendez2017web} \cite{tuli2020telepresence} \cite{soares2017mobile} \cite{herring2013telepresence} \cite{ng2015cloud} \cite{michaud2007telepresence} \cite{tan2019toward} \cite{cesta2016long} \cite{monroy2017integrating} \cite{beno2018work} \cite{kristoffersson2013review}. The majority of telepresence systems are intended for use in an office setting, and other application areas with the elderly, in healthcare, and in research. Most of the work has focused on the hardware capabilities and features. However, we focus on the software platform itself that can run on any hardware with some adaptation in the hardware level. In terms of software, we have included a number of components to perform embodied AI tasks to give a flavour of cognitive intelligence to the telepresence scenario. The closest work is ENRICHME \cite{cocsar2020enrichme} that supports some simple software level cognitive features. However, we offer a significant shift towards complex and sophisticated embodied AI features that has been tested to work on a real robot in real life use cases as well.

In terms of the embodied AI tasks, individual efforts on the subtasks has recently gained focus of the research community - like cognitive navigation ~\cite{duan2022survey} and human-robot dialogue. A number of work on Speech based HRI in robots has focused on accessibility ~\cite{tsui2015accessible} and cloud infrastructure for HRI using speech ~\cite{ deuerlein2021human}, however the area of speech HRI for general purpose telepresence scenario has limited peer reviewed work.   In cognitive navigation, for the `PointGoal' problem, there exists some work that uses frontier based planners ~\cite{batinovic2021multi} ~\cite{chattopadhyay2021robustnav}. There has been some work on person following by robot like ~\cite{personFollow1}, ~\cite{cheng2019person}, however, our work gives control of the remote user to follow a person making it suitable for telepresence scenario; and introduces engineering contributions to make the task work in real world. In recent times, `ObjectNav' task has grabbed the attention of robotics research community ~\cite{banerjee2022object}. The initial work on Semantic Visual Navigation \cite{yang2018visual} uses scene priors learnt from standard image dataset. Their work uses Graph Convolutional Networks (GCNs) to embed prior knowledge into a Deep Reinforcement Learning framework and is based on Actor-Critic model. However that work lacked a concrete decision model when two or more objects are in same scene. The proposed method makes an improvement on the GCN based ObjectNav \cite{tatiya2021knowledge} by using trajectory data priors along with a learnt region-object joint embedding learned from a GCN trainig to perform the ObjectNav task, in the lines of ~\cite{kiran2022spatial}. We have presented comparative results with the end to end RL based ObjectNav -- SemExp \cite{chaplot2020object} to support the efficiacy of the approach. Other works based on RL uses Q-learning based Actor-Critic for single object~\cite{gireesh2022object} or multiple objects~\cite{gireesh2023sequence}. In terms of `AreaGoal' problem, there has not been much dedicated work that has happened apart from some work on scene graph analysis ~\cite{liu2021toward} to decide the region. Another work on robot navigation learning based on subroutines from egocentric perception ~\cite{kumar2020learning} shows an example run for AreaGoal task in `washroom' region. However, the work does not give away details in the AreaGoal task specifically, neither did any standard benchmark studies on the AreaGoal task. Their work was more focussed on the PointGoal task. In contrast, our paper tackles the AreaGoal problem in great detail backed by results. Hence, this paper, as a first, has presented a novel methodology to tackle the problem. The combination of multiple software features within the telepresence framework is a unique proposition of this work, which is further evident from the comparative table~\ref{tab:comparison_variations}.


==> system.tex <==
\section{System architecture}

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figs/5_Combined_Architecture.png}
    \caption{A high-level system architecture of \system showing distributed set of building blocks spread across four entities -- master device, cloud server, robot, and robot-edge.}
    \label{fig:archi_high_level}
\end{figure*}

In this section, we provide a high-level overview of \system (Fig.~\ref{fig:archi_high_level}), which comprises of four major subsystems -- Communication, Cognitive Dialogue Exchange, Cognitive Navigation and User Interface. 

The telepresence system maintains a real-time connection with an application at the caregiver’s end and acts as an Avatar of the care giver at the patient’s premise. The caregiver must navigate the patient’s premise in real-time through the Avatar based on the audio-visual feedback. The care giver can provide a remote verbal instruction to the robot to navigate near a desired location inside the room (e.g., `bedroom'). The speech based human-robot interface understands the desired goal from the voice. Based on the in-situ analysis of the semantic map derived from the live captured frames, the robot is able to move to a position near to the intended location. Once the robot reaches near that position, the caregiver can take manual control and perform finer control through on-screen navigation buttons. The robot is connected with the caregiver’s mobile device over the Internet through a WebRTC based communication protocol. Navigation, though natural to humans is non-trivial for robots. The ‘PointGoal’ problem was solved using the egocentric views obtained from the robot, which are then combined to make a global view of the environment using a spatial transform. The global top-view map is then used to plan a trajectory using the A* planner. The ‘ObjectGoal’ and ‘AreaGoal’ problem has been solved by building a model on top of Graph Neural Network (GCN) based learning of trajectory paths and spatial relations between regions (areas) and objects of indoor scenes. Evaluation is based on path predicted based on similarity of visible regions, walk history and learned model. The Dialogue engine helps in disambiguation of tasks instructions specified verbally using a pre-trained model ‘wav2vec’, which is passed on to task identifier to understand the goal and invoke the corresponding task module as a service.

